On Privatizing Equilibrium Computation in Aggregate Games over Networks

We propose a distributed algorithm to compute an equilibrium in aggregate games where players communicate over a fixed undirected network. Our algorithm exploits correlated perturbation to obfuscate information shared over the network. We prove that our algorithm does not reveal private information of players to an honest-but-curious adversary who monitors several nodes in the network. In contrast with differential privacy based algorithms, our method does not sacrifice accuracy of equilibrium computation to provide privacy guarantees.

==> proofsOld.tex <==
%!TEX root = root.tex

\section{Proof of Theorem \ref{Th:Main}} \label{Sec:proofs}
%In Section \ref{Sec:PrivacyProof}, we show that our algorithm is private. In Section \ref{Sec:ConvergenceProof}, we sketch the proof that the iterates of the algorithm converge to the Nash equilibrium asymptotically. Details are omitted due to space limitations.

%----

\subsection{Proving Algorithm \ref{Algo:PrivDNEComp} is Private} \label{Sec:PrivacyProof}

Recall that $\Gfrak(\Acal^c)$ is the graph over non-adversarial nodes $\Acal^c$. Suppose $\Acal^c$ has $M$ nodes.
Let $I, J$ be two players in $\Acal^c$ and
$$F:={(f_i, \Xcal_i)}_{i \in \Vcal}, \quad \tilde{F} :={(\tilde{f}_i, \tilde{\Xcal}_i)}_{i \in \Vcal},$$
be two games in $\Fcal$ such that $\tilde{F}$ is identical to $F$, except that costs and strategy sets of players $I$ and $J$ are switched: 
$$ \tilde{f}_I = f_J, \ \tilde{f}_J = f_I, \ \tilde{\Xcal}_I = \Xcal_J, \ \tilde{\Xcal}_J = \Xcal_I.$$
For convenience, define $\pi: \Vcal \to \Vcal$ as the permutation that encodes the switch, i.e., 
$$\pi(I) = J, \ \pi(J)=I, \text{ and } \pi(i)=i \text{ for all } i \neq I,J.$$ 

Consider the execution of Algorithm \ref{Algo:PrivDNEComp} on $F$, given by
\begin{align*}
{\Esf}(F, \v{r}, {x}^0) := \{(x^k_i, v^k_i, \hat{v}^k_i) \text{ for } i \in \Vcal, k\geq 0 \},
\end{align*} 
with obfuscation sequence $\v{r}$ used in \eqref{Eq:PrivateAlgo1}, initialized with $x^0 \in \cap_{i=1}^N \Xcal_i$. We prove that there exists an obfuscation sequence $\v{\tilde{r}}$ such that execution ${\Esf}(\tilde{F}, \v{\tilde{r}}, x^0)$ of Algorithm \ref{Algo:PrivDNEComp} on $\tilde{F}$ with $\v{\tilde{r}}$ starting from $x^0$, is identical to ${\Esf}(F, \v{r}, x^0)$, from ${\Asf}$'s perspective. 
An arbitrary permutation over $\Acal^c$ is equivalent to a composition of a sequence of switches among two players in $\Acal^c$. As a result, the algorithm execution on games in $\Fcal$ can be made to appear identical from ${\Asf}$'s standpoint, proving the privacy of Algorithm \ref{Algo:PrivDNEComp}.


In the rest of the proof, we show how to construct $\v{\tilde{r}}$ that ensures ${\Esf}(\tilde{F}, \v{\tilde{r}}, x^0)$ and ${\Esf}(F, \v{r}, x^0)$ appear identical to ${\Asf}$.

Adversary observes $\{x^k_j, v^k_j, \hat{v}^k_j\}$ for all $j\in\Acal$ at each $k\geq0$. Consequently, perturbations utilized by corrupted nodes $j\in\Acal$ are same in both executions,
\begin{align}
\tilde{r}^k_{ji} = r^k_{ji} \text{ for all } j\in\Acal.
\label{eq:q.r}
\end{align}

%\noindent 
Moreover, ${\Asf}$ observes $\hat{v}^k_j$ for all $j\in\Acal$ and hence, all messages received by $j\in\Acal$ from $i\in\Acal^c$, denoted by $v^k_{ij}$, are identical for both executions, i.e., 
\begin{align}
\begin{aligned}
 \tilde{v}^k_{ij} = {v}^k_{ij} 
& \iff \tilde{v}^k_i + \alpha^k \tilde{r}^k_{ij} = v^k_i + \alpha^k r^k_{ij}  \\
& \iff \alpha^k \tilde{r}^k_{ij} = v^k_i + \alpha^k r^k_{ij} - \tilde{v}^k_i. %= v^k_j + \alpha^k r^k_{ji} - v^k_{\pi(j)}
\end{aligned}
\label{eq:v.v}
\end{align}
Adversary observes $\bar{x}^k$ for each $k\geq 0$. Enforcing
$$\tilde{x}^k_i = x^k_{\pi(i)}, \ \tilde{v}^k_i = v^k_{\pi(i)}, \ \hat{\tilde{v}}^k_i = \hat{v}^k_{\pi(i)},$$
results in $\bar{\tilde{x}}^k=\bar{x}^k$. 
%and ${\Asf}$ is unable to differentiate between games $F$, $\tilde{F}$. 
We have 
\begin{align}
&\hat{\tilde{v}}^k_i = \hat{v}^k_{\pi(i)} \nonumber \\
& \iff \sum_{j\in\Ncal_i} W_{ij} (\tilde{v}^k_j +\alpha^k \tilde{r}^k_{ji}) = \sum_{j \in \Ncal_{\pi(i)}} W_{\pi(i)j} (v^k_j +\alpha^k r^k_{j \pi(i)}) \nonumber \\
& \iff \sum_{j\in\Ncal_i \cap \Acal^c} \tilde{r}^k_{ji} = \frac{1}{\alpha^k \delta} \sum_{j \in \Ncal_{\pi(i)}} W_{\pi(i)j} (v^k_j +\alpha^k r^k_{j\pi(i)})  \nonumber \\
&  \qquad \qquad  - \frac{1}{\alpha^k \delta}\sum_{j\in\Ncal_i} W_{ij} {v}^k_{\pi(j)}  - \sum_{j\in \Ncal_i \cap \Acal} \tilde{r}^k_{ji}. \label{Eq:Constraint3}%
\end{align}%

%\item 
The obfuscation used by each player $i\in\Acal^c$ is locally balanced, and hence, we have
\begin{align}
 \sum_{j \in \Ncal_i} \tilde{r}^k_{ij} = 0 
 \iff \sum_{j \in \Ncal_i \cap \Acal^c} \tilde{r}^k_{ij} = - \sum_{j \in \Ncal_i \cap \Acal} \tilde{r}^k_{ij}. \label{Eq:Constraint4}%
\end{align}%
Let $\gamma$ be a vector of $\tilde{r}^k_{ij}$'s for $i,j\in\Acal^c$. In the sequel, let $\bone$ denote a vector of ones of appropriate dimension. For graph $\Gfrak(\Acal^c)$, define its oriented incidence matrix $B$, adjacency matrix $A$, degree matrix $D$, and the normalized graph Laplacian matrix $L$ as 
\begin{align*}
&B_{ij} = \begin{cases}
1, & \text{if node }i \text{ is head of edge }j,    \\
-1, & \text{if node }i \text{ is tail of edge }j, \\
0, &\text{otherwise},
\end{cases} \\
&A_{ij} = 
\begin{cases} 
1, & \text{if } (i,j) \text{ is edge in } \Gfrak(\Acal^c), \\
0, & \text{otherwise},
\end{cases} \\
&D = \diag(A \bone), \text{ and } L = I - D^{-1/2} A D^{-1/2}.%
\end{align*}%
Using the notation $z_+ \coloneqq \max\{z, 0\}$ and $z_- \coloneqq z_+ - z$ for a scalar $z$, define $B_+$ and $B_-$ as the matrices obtained from $B$, applying the respective operator componentwise.
Then, \eqref{Eq:Constraint3} - \eqref{Eq:Constraint4} can be written as
\begin{align*}
\underbrace{\begin{pmatrix} B_- & B_+ \\ B_+ & B_-\end{pmatrix}}_{:=T} \gamma = \underbrace{\begin{pmatrix} \xi^1 \\ \xi^2\end{pmatrix}}_{:=\xi} ,
\end{align*}
%where, $T^1$ and $T^2$ are boolean matrices with $N-\tau$ rows each, defined as 
%\begin{align*}
%    T^1_{im} &= \begin{cases}
%    1,  & \text{if $m^{th}$ entry of }  \gamma \text{ is } \tilde{r}^k_{ti}, \text{ for any } t\in \Acal^c, \\
%    0,  & \text{otherwise, } 
%    \end{cases} \\
%    T^2_{im} &= \begin{cases}
%    1,  & \text{if $m^{th}$ entry of }  \gamma \text{ is } \tilde{r}^k_{it}, \text{ for any } t\in \Acal^c, \\
%    0,  & \text{otherwise. } 
%    \end{cases} 
%\end{align*}
We prove that, 
\begin{align}
\rank T = \rank (T \ | \ \xi) = 2M - 1,
\label{eq:rankCond}
\end{align}
to show that $T\gamma=\xi$ admits at least one solution.

Notice that 
 \begin{align}
 \begin{aligned}
( \bone^\T \ | \ -\bone^\T )
  \begin{pmatrix} B_- & B_+ \\ B_+ & B_-\end{pmatrix}
% & = 
%\left( \bone^\T [B_- - B_+] \ | \ \bone^\T [B_+ - B_-] \right) \\
  = 
 \left( - \bone^\T B \ | \ \bone^\T B \right) = 0,
 \end{aligned}
 \label{eq:T.not.indep}
 \end{align}
proving that rows of $T$ are not linearly independent. Next, we show that $\rank T \geq 2M-1$. To that end, we have
\begin{align}
\rank T
&= \rank (T T^\T) \nonumber \\
&= \rank \begin{pmatrix} 
B_- B_-^\T + B_+ B_+^\T &\; B_- B_+^\T + B_+ B_-^\T \\ 
B_+ B_-^\T + B_- B_+^\T &\; B_- B_-^\T + B_+ B_+^\T\end{pmatrix} \nonumber \\
&\stackrel{(a)}= \rank \begin{pmatrix} 
D & A \\ 
A & D \end{pmatrix} \nonumber \\
&= \rank D + \rank (D - A D^{-1}A) \nonumber \\
&= M +  \rank (I_M - D^{-1/2}A D^{-1}A D^{-1/2}) \nonumber \\
&= M +  \rank (I_M - (I_M-L)^2) \nonumber \\
&= M +  \rank (2L - L^2) \nonumber \\
&\stackrel{(b)}\geq M +  \underbrace{\rank L}_{=M-1} + \rank (2I_M - L) - M \nonumber \\
&\stackrel{(c)}= M - 1 + \rank(2 I_M - L) \nonumber \\
&= 2M-1, \label{eq:rankT}
\end{align}
where $I_M$ is the $M \times M$ identity matrix.
Here, (a) follows from the definition of $B_+, B_-, D, A$, (b) follows from Sylvester's nullity theorem (see \cite{horn2012matrix}) and the fact that the rank of graph Laplapcian for the connected graph $\Gfrak(\Acal^c)$ on $M$ nodes is $M-1$. Furthermore, since $\Gfrak(\Acal^c)$ is not bipartite, the eigenvalues of $L$ are strictly less than 2, according to Lemma 1.7 in \cite{chung1997spectral}. Therefore, we have $\rank(2 I - L) = M$ that implies (c). Thus, \eqref{eq:T.not.indep} and \eqref{eq:rankT} together yield $\rank  T = 2M-1$. 





For the augmented matrix $(T \ | \ \xi)$, we have
\begin{align}
2 M - 1 \ \leq \ \rank( T \ | \ \xi ) \ \leq \ 2M. \label{Eq:Proof1} 
\end{align}
In the above relation, the inequality on the left follows from our earlier proof that $\rank T  = 2M-1$. The one on the right follows from the fact that the augmented matrix has $2M$ rows. We demonstrate that rows of $( T \ | \ \xi)$ are linearly dependent to conclude \eqref{eq:rankCond}. From \eqref{eq:T.not.indep}, we deduce
\begin{align*}
\left(\bone^\T \  | \ - \bone^\T \right) ( T \ | \ \xi) 
%&= \left( \bone^\T T^1 - \bone^\T T^2 \ | \ \bone^\T \xi^1 - \bone^\T \xi^2 \right)\\
&= \left( 0 \ | \ \bone^\T \xi^1 - \bone^\T \xi^2 \right).
\end{align*}
Now, we show $\bone^T \xi^1 - \bone^T \xi^2 = 0$ to conclude the proof. In the following, $| \Zcal |$ computes the cardinality of a set $\Zcal$.
\begin{small}
\begin{align*}
&\bone^T \xi^1 - \bone^T \xi^2   \\
&=  \frac{1}{\alpha^k \delta} \sum_{i\in\Acal^c} \sum_{j \in \Ncal_{\pi(i)}} W_{\pi(i)j} (v^k_j +\alpha^k r^k_{j\pi(i)})  \nonumber \\
&\qquad  - \frac{1}{\alpha^k \delta}\sum_{i\in\Acal^c}\sum_{j\in\Ncal_i} W_{ij} {v}^k_{\pi(j)}  - \sum_{i\in\Acal^c} \sum_{j\in \Ncal_i \cap \Acal} \tilde{r}^k_{ji} + \sum_{i\in\Acal^c} \sum_{j \in \Ncal_i \cap \Acal} \tilde{r}^k_{ij}\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
&\stackrel{(a)}{=}  \frac{1}{\alpha^k \delta} \sum_{i\in\Acal^c} \left[ \sum_{j \in \Ncal_{\pi(i)}} W_{\pi(i)j} v^k_j - \sum_{j\in\Ncal_i} W_{ij} {v}^k_{\pi(j)} \right]  \nonumber \\ %
&\qquad + \sum_{i\in\Acal^c} \sum_{j \in \Ncal_{\pi(i)}}  r^k_{j\pi(i)} - \sum_{i\in\Acal^c} \sum_{j\in \Ncal_i \cap \Acal} \tilde{r}^k_{ji} + \sum_{i\in\Acal^c} \sum_{j \in \Ncal_i \cap \Acal} \tilde{r}^k_{ij}\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
&\stackrel{(b)}{=}  \frac{1}{\alpha^k \delta} \sum_{i\in\Acal^c} \left[ \sum_{j \in \Ncal_{\pi(i)}} W_{\pi(i)j} v^k_j  - \sum_{j\in\Ncal_i} W_{ij} {v}^k_{\pi(j)} \right] \nonumber \\
&\qquad + \sum_{i\in\Acal^c} \sum_{j \in \Ncal_i\cap\Acal^c} r^k_{ji} + \sum_{i\in\Acal^c} \sum_{j \in \Ncal_i \cap \Acal} \tilde{r}^k_{ij}\\ 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%& (\text{Recall, } \tilde{r}^j_{ji} = r^k_{ji}, \ i \in\Acal^c, j\in\Acal \\
%&\quad \text{ and } \alpha^k \tilde{r}^k_{ij} = v^k_{i} + \alpha^k r^k_{ij} - v^k_{\rho(i)} \text{ if }  i \in \Acal^c, j \in \Acal)\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
&\stackrel{(c)}{=}  \frac{1}{\alpha^k \delta} \sum_{i\in\Acal^c} \left[ \sum_{j \in \Ncal_{\pi(i)}} W_{\pi(i)j} v^k_j  - \sum_{j\in\Ncal_i} W_{ij} {v}^k_{\pi(j)} \right] \nonumber \\
& \qquad + \sum_{i\in\Acal^c} \sum_{j \in \Ncal_{i}\cap\Acal^c} r^k_{ji} + \sum_{i\in\Acal^c} \sum_{j\in\Ncal_i\cap\Acal} \left[\frac{1}{\alpha^k}(v^k_i - v^k_{\pi(i)}) + r^k_{ij} \right] \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
&\stackrel{(d)}{=}  \underbrace{\frac{1}{\alpha^k \delta} \sum_{i\in\Acal^c} \left[ \sum_{j \in \Ncal_{\pi(i)}} W_{\pi(i)j} v^k_j  - \sum_{j\in\Ncal_i} W_{ij} {v}^k_{\pi(j)} \right]}_{Q_1} \nonumber \\
& \qquad  + \underbrace{\sum_{i\in\Acal^c} \sum_{j\in\Ncal_i\cap\Acal} \left[\frac{1}{\alpha^k}(v^k_i - v^k_{\pi(i)}) \right]}_{Q_2} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%&=  \sum_{i\in\Acal^c} \frac{1}{\alpha^k \delta}\sum_{j\in \Ncal_i} W_{ij} \left[ (v^k_j - v^k_{\rho(j)}) \right] + \sum_{i\in\Acal^c} \sum_{j\in \Ncal_i \cap \Acal^c} r^k_{ji} \\
%&\qquad  + \sum_{i\in\Acal^c} \sum_{j\in\Ncal_i\cap\Acal} \left[\frac{1}{\alpha^k}(v^k_i - v^k_{\rho(i)}) + r^k_{ij} \right], \\
%& \left( \text{Recall } \sum_{i\in\Acal^c} \sum_{j\in\Ncal_i\cap \Acal^c} r^k_{ij} + \sum_{i\in\Acal^c} \sum_{j\in\Ncal\cap\Acal} r^k_{ij} = 0 \right) \\
%&= \frac{1}{\alpha^k} \sum_{i\in\Acal^c} \left[  \frac{1}{\delta}\sum_{j\in \Ncal_i} W_{ij} (v^k_j - v^k_{\rho(j)}) + \sum_{j\in\Ncal_i\cap\Acal} (v^k_i - v^k_{\rho(i)})\right],\\
%&(\text{Recall } \rho(i) = i, \forall i \neq I,J, \ \& \ \rho(I) = J, \rho(J) = I)\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
&\stackrel{(e)}{=} \frac{1}{\alpha^k}\left(|\Ncal_I \cap \Acal^c \setminus I|+|\Ncal_I \cap \Acal|+ \frac{1-(|\Ncal_I|-1)\delta}{\delta}\right)(v^k_I - v^k_J )\\
&\qquad +\frac{1}{\alpha^k} \left(|\Ncal_J \cap \Acal^c \setminus J| + |\Ncal_J \cap \Acal| + \frac{1-(|\Ncal_J|-1)\delta}{\delta} \right)(v^k_J - v^k_I) \\
& = 0.
\end{align*}%
\end{small}%
We obtain (a) by rearranging terms and using $r^k_{ii}=0$ and $W_{ij} = \delta$, when, $(i,j)\in\Ecal$. We get (b) by writing, 
\begin{align*}
\sum_{i\in\Acal^c} \sum_{j \in \Ncal_{\pi(i)}}  r^k_{j\pi(i)} &= \sum_{i\in\Acal^c} \sum_{j \in \Ncal_i}  r^k_{ji} \\
&= \sum_{i\in\Acal^c} \sum_{j \in \Ncal_i\cal\Acal^c}  r^k_{ji} + \sum_{i\in\Acal^c} \sum_{j \in \Ncal_i \cap \Acal}  r^k_{ji},
\end{align*}
and using $r^k_{ji} = \tilde{r}^k_{ji}$, for all $j\in\Acal$ from \eqref{eq:q.r}. We use \eqref{eq:v.v} and replace $\tilde{r}^k_{ij}$, when, $i\in\Acal^c$ and $j\in\Acal$ to get equality (c). We get (d) by observing,
\begin{small}
\begin{align*}
\sum_{i\in\Acal^c} \left( \sum_{j\in\Ncal_i\cap\Acal^c} r^k_{ji} +\sum_{j\in\Ncal_i\cap\Acal} r^k_{ij}\right) = 0,%
\end{align*}%
\end{small}%
which is a consequence of \eqref{Eq:Constraint4}, i.e, adding all perturbations used by all players in $\Acal^c$ gives zero (balanced design of perturbations). Finally, we use the definition of permutation $\pi$ to simplify term $Q_1$,
\begin{small}
\begin{align*}
Q_1 &= \frac{1}{\alpha^k}\sum_{i\in\Acal^c} |\Ncal_i\cap\Acal| (v^k_i - v^k_{\pi(i)}) \\
&= \frac{1}{\alpha^k}|\Ncal_I \cap \Acal| (v^k_I - v^k_J) + \frac{1}{\alpha^k}|\Ncal_J \cap \Acal| (v^k_J - v^k_I).%
\end{align*}%
\end{small}%
And similarly for term $Q_2$, recall, $\pi(i)=i$, $\forall \ i \neq I,J$, 
\begin{small}
\begin{align*}
Q_2 &=\frac{1}{\alpha^k \delta} \sum_{i\in\Acal^c} \left[ \sum_{j \in \Ncal_{\pi(i) \cap \Acal^c}} W_{\pi(i)j} v^k_j  - \sum_{j\in\Ncal_i \cap \Acal^c} W_{ij} {v}^k_{\pi(j)} \right]\\
&= \frac{1}{\alpha^k \delta} \sum_{i\in\Acal^c} \left[(1-(|\Ncal_i|-1)\delta) v^k_i + \sum_{j\in\Ncal_i\setminus i} \delta v^k_j\right]\\
&\quad - \frac{1}{\alpha^k \delta} \sum_{i\in\Acal^c}\left[(1-(|\Ncal_i|-1)\delta) v^k_{\pi(i)} + \sum_{j\in\Ncal_i\setminus i} \delta v^k_{\pi(j)}\right] \\
&= \frac{1}{\alpha^k}\sum_{i\in\Acal^c} \left[\frac{(1-(|\Ncal_i|-1)\delta)}{\delta} (v^k_i - v^k_{\pi(i)})  +  \sum_{j\in\Ncal_i\setminus i} v^k_j- v^k_{\pi(j)}\right] \\
&= \frac{1}{\alpha^k}\left[ |\Ncal_I \cap \Acal \setminus I| + \frac{(1-(|\Ncal_I|-1)\delta)}{\delta}\right](v^k_I - v^k_J) \\
&\quad + \frac{1}{\alpha^k}\left[|\Ncal_J \cap \Acal \setminus J| + \frac{(1-(|\Ncal_J|-1)\delta)}{\delta}\right](v^k_J - v^k_I) %
\end{align*}%
\end{small}%
The expressions for $Q_1$ and $Q_2$ along with the fact that $|\Ncal_I \cap \Acal| + |\Ncal_I \cap \Acal^c \setminus I| = |\Ncal_I|-1$ we get equality (e), which, is quite clearly zero. This completes the proof of privacy of our algorithm. $\hfill \qed$




%\noindent \textasteriskcentered { \underline{Necessity of $\kappa(G) \geq \tau + 2$.}}
%We prove necessity via contradiction. We assume $\kappa(\Gfrak) = \tau+1$ and we have $\kappa(\Hcal)\geq 1$. 
%Consider $\Gfrak$ and adversarial corruption, such that $\kappa(\Hcal) = 1$ and $\Hcal$ is a tree (e.g. Fig.~\ref{Fig:Proof1}(Right)). Consider a leaf of graph $\Hcal$ denoted by $i$ and its parent node $I$. Consider a 2-switch $\pi$, such that $\pi(I)=J$ and $\pi(J)=I$ for some $J\in\Acal^c$; and games $F$, $\tilde{F}$ corresponding to permutation $\pi$. Consider executions ${\Esf}(F, \v{r}, {x}^0)$, ${\Esf}(\tilde{F}, \v{q}, {x}^0)$ as defined in sufficiency proof above. We focus on designing perturbation $\tilde{r}^k_{iI}$, such that algorithm execution lead to same observations by ${\Asf}$. 
%\begin{itemize}
%\item Since, $i$ is a leaf node, it only has 1 neighbor in $\Hcal$ and other neighbors are adversaries. The perturbations $\tilde{r}^k_{it} = r^k_{it}$ for $t\in\Acal$ to ensure ${\Asf}$ observes $\tilde{v}^k_{it} = v^k_{it}$ $\forall \ t\in\Acal$. As sum of all perturbations used by $i$ is zero, we have $\tilde{r}^k_{iI} = - \sum_{l\in\Ncal_i\cap\Acal} \tilde{r}^k_{il}$, a fixed value. 
%\item We need $\tilde{r}^k_{iI}$ to be such that $\hat{\tilde{v}}^k_I = \hat{v}^k_J$ (see \eqref{Eq:Constraint3}) and depends on $v^k_I$, $v^k_J$ and $r^k_{tI}$ ($t \in \Ncal_I$). 
%\end{itemize}
%Constraints described above on variable $\tilde{r}^k_{iI}$ are not consistent leading to a contradiction. Implying $\nexists \; \tilde{r}^k_{ij}$, such that two executions ${\Esf}(F, \v{r}, {x}^0)$ and ${\Esf}(\tilde{F}, \v{q}, {x}^0)$ lead to same observations by ${\Asf}$. This contradiction proves the necessity of $\kappa(\Gfrak)>\tau+1$.
%$\hfill \qed$

%-----------------
